End-user Comprehension of Transfer Risks in Smart Contracts

Smart contracts are increasingly used in critical use cases (e.g., financial transactions). Thus, it is pertinent to ensure that end-users understand the transfer risks in smart contracts. To address this, we investigate end-user comprehension of risks in the most popular Ethereum smart contract (i.e., USD Tether (USDT)) and their prevalence in the top ERC-20 smart contracts. We focus on five transfer risks with severe impact on transfer outcomes and user objectives, including users being blacklisted, contract being paused, and contract being arbitrarily upgraded. Firstly, we conducted a user study investigating end-user comprehension of smart contract transfer risks with 110 participants and USDT/MetaMask. Secondly, we performed manual and automated source code analysis of the next top (78) ERC-20 smart contracts (after USDT) to identify the prevalence of these risks. Results show that end-users do not comprehend real risks: most (up to 71.8% of) users believe contract upgrade and blacklisting are highly severe/surprising. More importantly, twice as many users find it easier to discover successful outcomes than risky outcomes using the USDT/MetaMask UI flow. These results hold regardless of the self-rated programming and Web3 proficiency of participants. Furthermore, our source code analysis demonstrates that the examined risks are prevalent in up to 19.2% of the top ERC-20 contracts. Additionally, we discovered (three) other risks with up to 25.6% prevalence in these contracts. This study informs the need to provide explainable smart contracts, understandable UI and relevant information for risky outcomes.

==> implementation.tex <==
\section{Research Methodology}
\label{sec:method}

\subsection{Retrieving source code}
% \addfig{source-code-methodology}{Retrieval of source code for most-used ERC-20 smart contracts.}

We analyzed all Ethereum transactions from Mar-22-2022 04:36:03AM UTC (block 14434001) to Jun-23-2022 10:03:37AM UTC (block 15012398) to retrieve the most transacted with 79 ERC-20 contracts used during that period. Details on the processing can be found in \autoref{fig:source-code-methodology}.


\subsection{Examining Top Contracts}
For our analysis period, the ERC-20 USDT contract accounted for over 60\% of the transactions among the 364 smart contracts which were most transacted with.

We then examined the source code to extract unexpected elements that may contradict user expectations.

\subsection{Unexpected Features in USDT Smart Contract}
The following are features present in the USDT smart contract that are not detailed in the ERC-20 token standard \cite{ERC20TokenStandard} which we deem as unexpected.
\begin{itemize}
	\item \textbf{Contract Pause capability}. The contract owner (currently a multi-signature wallet, which presumably is controlled by Tether Limited) may unilaterally pause and resume all transfers of USDT among users.
	\item \textbf{User Blacklist capability}. The contract owner may unilaterally blacklist users, thus banning them from using their funds. According to analytics \cite{USDTBannedAddresses}, 914 addresses are currently blacklisted, totalling an inaccessible amount of 469,679,412 USDT.
	\item \textbf{Contract Upgrade capability}. The contract owner may unilaterally upgrade the current smart contract to an arbitrary new smart contract, forwarding all transfer calls to the new contract. This capability has not yet been utilized.
	\item \textbf{Transfer Fee Increase capability}. The contract owner may unilaterally increase a transfer fee by updating parameters on the smart contract. This fee is currently set to 0, and its increase is limited to the minimum value of 0.19\% and 49 USDT.
\end{itemize}

\subsection{Examining Other ERC-20 Contracts}
In order to examine the generalizability of these features to other ERC-20 contracts, we extracted top ERC-20 smart contracts from our pool of 364 smart contracts with source code using the methodology in \autoref{fig:source-code-methodology}. This yielded 78 additional ERC-20 contracts.

==> revision1.tex <==
\title{Revision 1 Response}
% \maketitle

\renewcommand{\thetable}{\Roman{table}}
\renewcommand{\thesection}{\Roman{section}}
\pagenumbering{roman}

% Reviewer tags
\newcommand{\ra}{{\colorbox{magenta}{\textcolor{white}{Reviewer A}}}}
\newcommand{\rb}{{\colorbox{blue}{\textcolor{white}{Reviewer B}}}}
\newcommand{\rc}{{\colorbox{orange}{\textcolor{white}{Reviewer C}}}}
\newcommand{\mr}{{\colorbox{gray}{\textcolor{white}{Meta Reviewer}}}}
% quote
\newcommand{\q}[2]{
    \noindent #1 \textit{"#2"}
}

\newcommand{\res}{
    \vspace{0.1cm}
    \hrule
    \vspace{0.3cm}
}

\newcommand{\ip}[1]{\textcolor{brown}{#1}}

\newcommand{\yhref}[2]{
    \href{#1}{\textcolor{blue}{#2}}
}

\newpage
\clearpage



{\huge \textbf{Revision Response}}

\todo Once finalized, duplicate the meta-reviewer points into the relevant letter reviewers (e.g. meta-reviewer point may be based on reviewer A's point. In this case, duplicate it into reviewer A, since this has not yet been done.)

We thank all reviewers for the 
%Thank you for your 
detailed reviews and insightful comments.
\begin{itemize}
    \item We have broken down the action points by reviewer for your convenience (so that you may refer directly to your section).
    \item We have colored all \ip{direct quotes from the paper itself in brown.}
\end{itemize}

Here are direct links to the sections by reviewer:
\begin{itemize}
\item \mr: \autoref{rev1:mr}
\item \ra: \autoref{rev1:ra}
\item \rb: \autoref{rev1:rb}
\item \rc: \autoref{rev1:rc}
\end{itemize}

\twocolumn
\input{revision1/meta-reviewer.tex}
\input{revision1/reviewer-a.tex}
\input{revision1/reviewer-b.tex}
\input{revision1/reviewer-c.tex}



\newpage
\clearpage

\pagenumbering{arabic}
\setcounter{page}{1}
\setcounter{table}{1}
\setcounter{section}{1}

\renewcommand{\thetable}{\arabic{table}}
\renewcommand{\thesection}{\arabic{section}}
